Evaluating Vision-Language Models for Emotion Recognition

Large Vision-Language Models (VLMs) have achieved unprecedented success in several objective multimodal reasoning tasks. However, to further enhance their capabilities of empathetic and effective communication with humans, improving how VLMs process and understand emotions is crucial. Despite significant research attention on improving affective understanding, there is a lack of detailed evaluations of VLMs for emotion-related tasks, which can potentially help inform downstream fine-tuning efforts. In this work, we present the first comprehensive evaluation of VLMs for recognizing evoked emotions from images. We create a benchmark for the task of evoked emotion recognition and study the performance of VLMs for this task, from perspectives of correctness and robustness. Through several experiments, we demonstrate important factors that emotion recognition performance depends on, and also characterize the various errors made by VLMs in the process. Finally, we pinpoint potential causes for errors through a human evaluation study. We use our experimental results to inform recommendations for the future of emotion research in the context of VLMs.

==> latex/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we present the first extensive evaluation of popular vision-language models for the task of evoked emotion recognition. We first introduce a sizeable and representative benchmark for the task. Using several probing strategies, we study how well VLMs perform emotion recognition zero-shot, including whether they display biases to certain emotions, are sensitive to perturbations in prompts, or are capable of self-reasoning for emotion prediction. We then analyze the different types of errors made by the models, and aim to identify potential causes through a human study. Finally, we include a broader discussion on the usage of VLMs for emotion-related tasks, and useful practices for emotion research, especially when releasing new datasets or benchmarks. We hope our study highlights the need 
